Convex Bounds on the Softmax Function with Applications to Robustness Verification

The softmax function is a ubiquitous component at the output of neural networks and increasingly in intermediate layers as well. This paper provides convex lower bounds and concave upper bounds on the softmax function, which are compatible with convex optimization formulations for characterizing neural networks and other ML models. We derive bounds using both a natural exponential-reciprocal decomposition of the softmax as well as an alternative decomposition in terms of the log-sum-exp function. The new bounds are provably and/or numerically tighter than linear bounds obtained in previous work on robustness verification of transformers. As illustrations of the utility of the bounds, we apply them to verification of transformers as well as of the robustness of predictive uncertainty estimates of deep ensembles.

==> Convex Bounds on the Softmax Function/ER.tex <==
\section{BOUNDS FROM EXPONENTIAL\\-RECIPROCAL DECOMPOSITION}
\label{sec:ER}

Previous work \citep{bonaert2021fast} took the natural approach of decomposing the softmax function \eqref{eqn:softmax} as the composition of a sum of exponentials, $q_1 = \se(\tx)$, 
%\[
%q_1 = \se(\tx) = 1 + \sum_{j=2}^K e^{\tx_j},
%\]
and the reciprocal function $p_1 = 1 / q_1$.\footnote{\citet{bonaert2021fast}'s use of the second form in \eqref{eqn:softmax} avoids a multiplication needed by \citet{Shi2020Robustness}.} They as well as \citet{Shi2020Robustness} derive lower and upper bounds on $\se(\tx)$ and $1/q_1$ that are affine in $x$ and $q_1$ respectively, and compose these bounds to obtain bounds on the softmax. We review the bounds of \citet{Shi2020Robustness,bonaert2021fast} in Section~\ref{sec:ER:lin}, combining their respective advantages, before starting to improve upon them in Section~\ref{sec:ER:non}.

\subsection{Existing Linear Bounds}
\label{sec:ER:lin}

\paragraph{Sum of Exponentials} For the sum of exponentials $\se(\tx)$, each exponential $e^{\tx_j}$ is a function of a scalar $\tx_j \in [\tl_j, \tu_j]$. By virtue of convexity and following \citet{Shi2020Robustness}, each exponential can be bounded from above by the chord between the endpoints $(\tl_j, e^{\tl_j})$ and $(\tu_j, e^{\tu_j})$, and from below by a tangent line passing through $(t_j, e^{t_j})$. The resulting bounds can be written as 
\begin{subequations}\label{eqn:lin_exp}
\begin{align}
    \se(\tx) &\geq 1 + \sum_{j=2}^K e^{t_j} (\tx_j - t_j + 1),\label{eqn:lin_expLB}\\
    \se(\tx) &\leq \olse(\tx; \tl, \tu)% 1 + \sum_{j=2}^K \left(\frac{\tu_j - \tx_j}{\tu_j - \tl_j} e^{\tl_j} + \frac{\tx_j - \tl_j}{\tu_j - \tl_j} e^{\tu_j}\right)
    ,\label{eqn:lin_expUB}
\end{align}
\end{subequations}
where 
\begin{equation}\label{eqn:tj}
t_j = \min\left\{\log\frac{e^{\tu_j} - e^{\tl_j}}{\tu_j - \tl_j}, \tl_j + 1 \right\}
\end{equation}
and we have defined the chordal upper bound on $\se(x)$, 
\begin{equation}\label{eqn:seUB}
    \olse(x; l, u) = \sum_{j=1}^K \left(\frac{u_j - x_j}{u_j - l_j} e^{l_j} + \frac{x_j - l_j}{u_j - l_j} e^{u_j}\right).
\end{equation}
In \eqref{eqn:tj}, the first choice of $t_j$ makes the slope $e^{t_j}$ in the lower bound \eqref{eqn:lin_expLB} equal to the corresponding slope in the upper bound \eqref{eqn:lin_expUB}, thus minimizing the area between them \citep{bonaert2021fast}. The second term in \eqref{eqn:tj} ensures that the lower bound \eqref{eqn:lin_expLB} is non-negative for all $\tx_j \in [\tl_j, \tu_j]$.\footnote{In this second case, we allow the slopes in \eqref{eqn:lin_expLB}, \eqref{eqn:lin_expUB} to be different, like \citet{Shi2020Robustness} and unlike \citet{bonaert2021fast}.} In \eqref{eqn:seUB}, we adopt the convention that if $l_j = x_j = u_j = 0$ (as is true for $\tl_1, \tx_1, \tu_1$), then the $j$th term in the sum is $1$.  

\paragraph{Reciprocal} The same approach is applied to the reciprocal $1/q_1$, which is also a convex function of a scalar. First we need lower and upper bounds on the input $q_1$ to the reciprocal. These are obtained by minimizing the lower bound \eqref{eqn:lin_expLB} and maximizing the upper bound \eqref{eqn:lin_expUB} over $\tx \in [\tl, \tu]$, resulting in
\begin{subequations}\label{eqn:lin_z}
\begin{align}
    \ulq_1^\lin &= 1 + \sum_{j=2}^K e^{t_j} (\tl_j - t_j + 1),\label{eqn:lin_zLB}\\
    \olq_1^\lin &= \se(\tu) = \frac{1}{\ulp_1}.\label{eqn:lin_zUB}
\end{align}
\end{subequations}
Then we have the following bounds on the reciprocal: %(after simplification):
\begin{align}\label{eqn:lin_recip}
    \frac{1}{t_{q_1}} \left(2 - \frac{q_1}{t_{q_1}}\right) \leq \frac{1}{q_1} \leq \frac{1}{\ulq_1^\lin} + \ulp_1 - \frac{\ulp_1 q_1}{\ulq_1^\lin},
\end{align}
where $t_{q_1} = \max\{\sqrt{\ulq_1^\lin \olq_1^\lin}, \olq_1^\lin/2 \}$ is the $q_1$ value of the tangent point.

\paragraph{Softmax} Overall bounds on the softmax output $p_1$ are obtained by composing bounds \eqref{eqn:lin_exp} and \eqref{eqn:lin_recip} with $q_1 = \se(\tx)$ and $p_1 = 1/q_1$. Specifically, upper bound \eqref{eqn:lin_expUB} is composed with the lower bound in \eqref{eqn:lin_recip} to yield the overall lower bound 
\begin{subequations}\label{eqn:lin}
\begin{align}\label{eqn:lin_LB}
    L^\lin(\tx) = &\frac{1}{t_{q_1}} \left(2 - \frac{\olse(\tx; \tl, \tu)}{t_{q_1}} \right). %\frac{1}{t_{q_1}} \left( 1 + \phantom{\sum_{j=2}^K} \right. \right.\nonumber\\
    %&\left. \left. \sum_{j=2}^K \left(\frac{\tu_j - \tx_j}{\tu_j - \tl_j} e^{\tl_j} + \frac{\tx_j - \tl_j}{\tu_j - \tl_j} e^{\tu_j}\right) \right) \right).
\end{align}
Similarly, the combination of \eqref{eqn:lin_expLB} and the upper bound in \eqref{eqn:lin_recip} yield 
\begin{equation}\label{eqn:lin_UB}
    U^\lin(\tx) = \frac{1}{\ulq_1^\lin} + \ulp_1 - \frac{\ulp_1}{\ulq_1^\lin} \left( 1 + \sum_{j=2}^K e^{t_j} (\tx_j - t_j + 1) \right).
\end{equation}
\end{subequations}

\subsection{New Nonlinear Bounds}
\label{sec:ER:non}

We now depart from \citet{Shi2020Robustness,bonaert2021fast} and derive nonlinear bounds on the softmax function using the same exponential-reciprocal decomposition. This is done by further exploiting the convexity of the functions 
$\se(\tx)$ and $1/q_1$. 

\paragraph{Sum of Exponentials} We now regard $q_1$ as an intermediate variable corresponding to the sum of exponentials $\se(\tx)$ but no longer bound by the strict equality $q_1 = \se(\tx)$. For a lower bound on $q_1$, we use $\se(\tx)$ itself, i.e., we relax $q_1 = \se(\tx)$ to 
\begin{equation}\label{eqn:ER_expLB}
    q_1 \geq \se(\tx).% = 1 + \sum_{j=2}^K e^{\tx_j}.
\end{equation}
Since $\se(\tx)$ is convex, the above constraint is in the desired form as in \eqref{eqn:LU}: it specifies a convex set of $(x, q_1)$ and is compatible with convex optimization. On the other hand, for an upper bound on $q_1$, we require a concave function of $x$. We thus reuse the upper bound \eqref{eqn:lin_expUB}, which is linear (and hence concave) in $x$.

\paragraph{Reciprocal} Similarly for the reciprocal where the exact relation is $p_1 = 1/q_1$, we use $1/q_1$ itself as the lower bound on $p_1$ %, $p_1 \geq 1/q_1$, 
and reuse the upper bound in \eqref{eqn:lin_recip}. For the latter however, it is possible to substitute a tighter lower bound on $q_1$ than $\ulq_1^\lin$ in \eqref{eqn:lin_zLB}. The reason is that we can now minimize the lower bound in \eqref{eqn:ER_expLB} over $\tx \in [\tl, \tu]$ instead of the one in \eqref{eqn:lin_expLB}, resulting in 
\begin{equation}\label{eqn:ER_zLB}
    \ulq_1^\ER = \se(\tl) = \frac{1}{\olp_1}. %\geq \ulq_1^\lin.
\end{equation}
The upper bound on $q_1$ is still $\olq_1^\lin$ \eqref{eqn:lin_zUB}. We therefore have %the bounds 
\begin{equation}\label{eqn:ER_recip}
    \frac{1}{q_1} \leq p_1 \leq \olp_1 + \ulp_1 - \olp_1 \ulp_1 q_1.
\end{equation}

\paragraph{Softmax} Overall bounds on the softmax are obtained by composing \eqref{eqn:ER_expLB}, \eqref{eqn:lin_expUB} with \eqref{eqn:ER_recip}, specifically the lower bound with the upper bound and vice versa. The results are 
\begin{subequations}\label{eqn:ER}
\begin{align}
    L^\ER(\tx) &= \frac{1}{\olse(\tx; \tl, \tu)}%\left( 1 + \sum_{j=2}^K \left(\frac{\tu_j - \tx_j}{\tu_j - \tl_j} e^{\tl_j} + \frac{\tx_j - \tl_j}{\tu_j - \tl_j} e^{\tu_j}\right) \right)^{-1}
    ,\label{eqn:ER_LB}\\
    U^\ER(\tx) &= \olp_1 + \ulp_1 - \olp_1 \ulp_1 \se(\tx).\label{eqn:ER_UB}
\end{align}
\end{subequations}
The lower bound $L^\ER(\tx)$ is a composition of $\olse(\tx; \tl, \tu)$, an affine function of $x$, with the reciprocal function. It is thus convex by the composition properties of convex functions \citep[Sec.~3.2.2]{boyd2004convex}. The upper bound $U^\ER(\tx)$ has a sum of exponentials with a negative multiplier in front and is hence concave, as desired.

\begin{theorem}\label{thm:ER_lin}
The nonlinear bounds $L^\ER(\tx)$, $U^\ER(\tx)$ are tighter than the linear bounds $L^\lin(\tx)$, $U^\lin(\tx)$:
\[
L^\lin(\tx) \leq L^\ER(\tx) \leq p_1 \leq U^\ER(\tx) \leq U^\lin(\tx) \quad \forall \tx \in [\tl, \tu].
\]
\end{theorem}
We defer all proofs to Appendix~\ref{sec:proofs}.


==> Convex Bounds on the Softmax Function/LSE.tex <==
\section{BOUNDS FROM LOG-SUM-EXP DECOMPOSITION}
\label{sec:LSE}

In this section, we depart from the exponential-reciprocal decomposition altogether and consider an alternative decomposition, obtained by taking the logarithm of the softmax \eqref{eqn:softmax}, $r_1 = -\lse(\tx)$,
and then exponentiating, $p_1 = e^{r_1}$. Here 
%\begin{equation}\label{eqn:lse}
$\lse(x) = \log\left( \sum_{j=1}^K e^{x_j} \right)$ 
%\end{equation}
is the ``log-sum-exp'' (LSE) function, a well-known convex function. Its negative $-\lse(\tx)$ is therefore concave in $x$.

We follow the same approach as in Section~\ref{sec:ER:non}, bounding the exponential and LSE functions and then composing the bounds. 

\paragraph{Exponential} For the exponential function $p_1 = e^{r_1}$, which is again a convex function of a scalar, we use $e^{r_1}$ itself as the lower bound on $p_1$ and a chord of the function as the upper bound. Noting that $\lse(\tx)$ is increasing in all inputs $\tx_j$, $r_1$ is bounded within the interval $[-\lse(\tu), -\lse(\tl)]$, and we may thus use the chord connecting the points $(-\lse(\tu), e^{-\lse(\tu)})$ and $(-\lse(\tl), e^{-\lse(\tl)})$. Using \eqref{eqn:const} to rewrite $-\lse(\tu)$, $-\lse(\tl)$ as $\log(\ulp_1)$, $\log(\olp_1)$, the bounds on $p_1$ in terms of $r_1$ are 
\begin{equation}\label{eqn:LSE_exp}
    e^{r_1} \leq p_1 \leq \frac{\log(\olp_1) - r_1}{\log(\olp_1) - \log(\ulp_1)} \ulp_1 + \frac{r_1 - \log(\ulp_1)}{\log(\olp_1) - \log(\ulp_1)} \olp_1.
\end{equation}

\paragraph{Log-Sum-Exp} For the log-sum-exp function $-\lse(\tx)$, since it is concave in $x$, we may use it as the \emph{upper} bound on its output $r_1$:
\begin{equation}\label{eqn:LSE_lseUB}
    r_1 \leq -\lse(\tx).
\end{equation}

It remains to find a lower bound on $-\lse(\tx)$ that is convex in $x$. In the case $K = 2$, $-\lse(\tx) = -\log(1 + e^{\tx_2})$ is a concave function of a scalar $\tx_2 \in [\tl_2, \tu_2]$ and we may bound it as before using the chord between endpoints,
\begin{multline}\label{eqn:LSE_lseLB2}
    -\log\left(1 + e^{\tx_2}\right) \geq -\frac{\tu_2 - \tx_2}{\tu_2 - \tl_2} \log\left(1 + e^{\tl_2}\right)\\ 
    - \frac{\tx_2 - \tl_2}{\tu_2 - \tl_2} \log\left(1 + e^{\tu_2}\right).
\end{multline}
This is linear and hence convex in $x$.

For $K > 2$, the challenge is that $-\lse(\tx)$ is a multivariate function. Here we provide two bounds with different strengths and weaknesses. In Appendix~\ref{sec:LSE:alt}, we describe a third bound that more directly extends the $K=2$ case \eqref{eqn:LSE_lseLB2} but turns out not to be as tight. For the first bound, we rewrite $-\lse(\tx)$ as $-\lse(\tx) = x_1 - \lse(x)$ so that $-\lse(x)$ is the non-convex part to be bounded. For this, we use chordal bounds on the exponentials similar to \eqref{eqn:lin_expUB}:
\begin{equation}\label{eqn:lseUB}
    \lse(x) %= \log\left( \sum_{j=1}^K e^{x_j} \right)
    \leq \log\left(\olse(x; l, u)\right).%\sum_{j=1}^K \left(\frac{u_j - x_j}{u_j - l_j} e^{l_j} + \frac{x_j - l_j}{u_j - l_j} e^{u_j}\right) \right).
\end{equation}
Hence
\begin{equation}\label{eqn:LSE_lseLB}
    -\lse(\tx) \geq x_1 - \log\left( \olse(x; l, u)\right).%\sum_{j=1}^K \left(\frac{u_j - x_j}{u_j - l_j} e^{l_j} + \frac{x_j - l_j}{u_j - l_j} e^{u_j}\right) \right).
\end{equation}
For the second bound, let $j^* = \argmax_j (l_j + u_j)$ be the index of the largest input in terms of the midpoints $m_j = (l_j + u_j) / 2$. Define the vector of differences $\dot{x}$, $\dot{x}_{j} = x_j - x_{j^*}$, $j = 1,\dots,K$, with corresponding lower and upper bounds $\dot{l}_j$, $\dot{u}_j$. %$l_{jj^*}$, $u_{jj^*}$. 
We then use the relation $\tx = \dot{x}%_{\cdot j^*} 
- \dot{x}_{1}$ and the translation property of LSE to write $-\lse(\tx) = \dot{x}_{1} - \lse(\dot{x}%_{\cdot j^*}
)$. By bounding $\lse(\dot{x}%_{\cdot j^*}
)$ using chordal bounds on exponentials as in \eqref{eqn:lseUB}, we obtain 
\begin{equation}\label{eqn:LSE_lseLB*}
    -\lse(\tx) \geq \dot{x}_{1} - \log\left(\olse(\dot{x}; \dot{l}, \dot{u})\right).%1 + \phantom{\sum_{j\neq j^*}} \right.
    %\\\left. \sum_{j\neq j^*} \left(\frac{u_{jj^*} - x_{jj^*}}{u_{jj^*} - l_{jj^*}} e^{l_{jj^*}} + \frac{x_{jj^*} - l_{jj^*}}{u_{jj^*} - l_{jj^*}} e^{u_{jj^*}}\right) \right).
\end{equation}
In both \eqref{eqn:LSE_lseLB} and \eqref{eqn:LSE_lseLB*}, since the term after $x_1$ or $\dot{x}_{1}$ is the composition of an affine function of $x$ with $-\log$, the right-hand sides of \eqref{eqn:LSE_lseLB}, \eqref{eqn:LSE_lseLB*} are convex functions of $x$ as desired. The advantage of \eqref{eqn:LSE_lseLB*} is that the inputs $\dot{x}_{j}$ to $\lse(\dot{x}%_{\cdot j^*}
)$ tend to be negative, thus placing them in the flatter parts of the exponentials $e^{\dot{x}_{j}}$ and leading to less loss when these exponentials are bounded by chords. The disadvantage of \eqref{eqn:LSE_lseLB*} is that the chords are over intervals $[\dot{l}_{j}, \dot{u}_{j}]$ that tend to be wider than the intervals $[l_j, u_j]$ used in \eqref{eqn:LSE_lseLB}.

\paragraph{Softmax} Overall bounds on the softmax are obtained by composing \eqref{eqn:LSE_lseUB} and \eqref{eqn:LSE_lseLB} or \eqref{eqn:LSE_lseLB*} with \eqref{eqn:LSE_exp}, this time matching lower bound with lower bound and upper with upper:
\begin{subequations}\label{eqn:LSE}
\begin{align}
    L^{\lse}(x) &= \frac{e^{x_1}}{\olse(x; l, u)}%e^{x_1} \left( \sum_{j=1}^K \left(\frac{u_j - x_j}{u_j - l_j} e^{l_j} + \frac{x_j - l_j}{u_j - l_j} e^{u_j}\right) \right)^{-1}
    ,\label{eqn:LSE_LB}\\
    L^{\lse*}(x) &= \frac{e^{\dot{x}_1}}{\olse(\dot{x}; \dot{l}, \dot{u})}%e^{x_{1j^*}} \left(1 + \phantom{\sum_{j\neq j^*}} \right.\nonumber\\
    %&\left. \sum_{j\neq j^*} \left(\frac{u_{jj^*} - x_{jj^*}}{u_{jj^*} - l_{jj^*}} e^{l_{jj^*}} + \frac{x_{jj^*} - l_{jj^*}}{u_{jj^*} - l_{jj^*}} e^{u_{jj^*}}\right) \right)^{-1}
    ,\label{eqn:LSE_LB*}\\
    %L^{\lse2}(x) &= e^{x_{1j^*}} \left(1 + \phantom{\sum_{j\neq j^*}} \right.\nonumber\\
    %&\left. \sum_{j\neq j^*} \left(\frac{u_{jj^*} - x_{jj^*}}{u_{jj^*} - l_{jj^*}} e^{l_{jj^*}} + \frac{x_{jj^*} - l_{jj^*}}{u_{jj^*} - l_{jj^*}} e^{u_{jj^*}}\right) \right)^{-1},\label{eqn:LSE_LB*}\\
    U^{\lse}(x) &= \frac{\ulp_1 \log(\olp_1) - \olp_1 \log(\ulp_1) - (\olp_1 - \ulp_1) \lse(\tx)}{\log(\olp_1) - \log(\ulp_1)}%\frac{\ulp_1 \log(\olp_1) - \olp_1 \log(\ulp_1)}{\log(\olp_1) - \log(\ulp_1)} - \frac{\olp_1 - \ulp_1}{\log(\olp_1) - \log(\ulp_1)} \lse(\tx)
    .\label{eqn:LSE_UB}
\end{align}
\end{subequations}
We use the lower bounds in \eqref{eqn:LSE_LB}, \eqref{eqn:LSE_LB*} for $K > 2$ and the upper bound \eqref{eqn:LSE_UB} for all $K$. Bound \eqref{eqn:LSE_LB*} is in fact a generalization of the ER lower bound \eqref{eqn:ER_LB} and coincides with \eqref{eqn:ER_LB} when $j^* = 1$. The lower bounds \eqref{eqn:LSE_LB}, \eqref{eqn:LSE_LB*} are the compositions of the right sides of \eqref{eqn:LSE_lseLB}, \eqref{eqn:LSE_lseLB*}, previously argued to be convex in $x$, with the exponential function, which is convex and increasing. Hence $L^{\lse}(x)$, $L^{\lse*}(x)$ are convex by the composition properties of convex functions \citep[Sec.~3.2.4]{boyd2004convex}. The upper bound $U^{\lse}(x)$ is concave in $x$ as it has $\lse(\tx)$ with a negative multiplier.

For an overall lower bound in the case $K = 2$, we take lower bound \eqref{eqn:LSE_lseLB2} instead of \eqref{eqn:LSE_lseLB} or \eqref{eqn:LSE_lseLB*} and exponentiate. %\eqref{eqn:LSE_lseLB0} instead of \eqref{eqn:LSE_lseLB} since $\lse(x_2^K) - x_1 = \tx_2$ and the upper bound \eqref{eqn:lse2UB} is not needed. After exponentiating \eqref{eqn:LSE_lseLB0} and 
After simplifying, this yields
\begin{equation}\label{eqn:LSE_LB2}
    L^{\lse_2}(x) = \left(\ulp_1\right)^{(\tx_2 - \tl_2) / (\tu_2 - \tl_2)} \Bigl(\olp_1\Bigr)^{(\tu_2 - \tx_2) / (\tu_2 - \tl_2)},
\end{equation}
which is an exponential function of $\tx_2$ and hence convex ($\lse_2$ indicates that this bound is only for $K = 2$).

\begin{theorem}\label{thm:LSE_ER}
The log-sum-exp upper bound $U^{\lse}(x)$ is tighter than the nonlinear exponential-reciprocal upper bound $U^\ER(x)$,
\[
p_1 \leq U^{\lse}(x) \leq U^\ER(x) \quad \forall x \in [l, u],
\]
for all $K \geq 2$. The log-sum-exp lower bound $L^{\lse_2}(x)$ is tighter than the nonlinear exponential-reciprocal lower bound $L^\ER(x)$,
\[
L^\ER(x) \leq L^{\lse_2}(x) \leq p_1 \quad \forall x \in [l, u],
\]
for $K=2$.
\end{theorem}
%The proof is provided in Appendix~\ref{sec:LSE:proof}.
%\begin{proof}[Proof sketch]
%To prove the inequality for the upper bounds, we rewrite both $U^\ER(x)$ and $U^{\lse}(x)$ as convex combinations of the constant bounds $\ulp_1$ and $\olp_1$. We then compare the coefficients in the two convex combinations to show that $U^{\lse}(x) \leq U^\ER(x)$.
%
%To prove the inequality for the lower bounds in the case $K=2$, we rewrite $L^\ER(x)$ as a weighted harmonic mean of $\ulp_1$ and $\olp_1$. We then recognize that $L^{\lse}(x)$ \eqref{eqn:LSE_LB2} is a weighted geometric mean of the same quantities with the same weights. The result follows from the inequality of (weighted) harmonic and geometric means.
%
%Detailed steps for both parts are in Appendix~\ref{sec:LSE:proof}.
%\end{proof}

For $K = 2$ inputs, the softmax function \eqref{eqn:softmax2} and all bounds (linear, ER, LSE) can be plotted as functions of the scalar $\tx_2$. We do so in Figure~\ref{fig:logistic_bounds} for the input interval $[\tl_2, \tu_2] = [-2, 2]$. In addition to confirming Theorems~\ref{thm:ER_lin} and \ref{thm:LSE_ER}, the figure shows that the gap between the ER lower bound $L^\ER$ and softmax is about twice as large as for the LSE lower bound $L^{\lse_2}$, and similarly for the upper bounds. While $L^\lin$ is tangent to $L^\ER$, $U^\lin$ exhibits a larger gap. These observations continue to hold for $K > 2$ in Section~\ref{sec:synth}.

\begin{figure}[th]
    \centering
    \includegraphics[width=0.85\columnwidth]{figures/logistic_bounds_aistats.pdf}
    \caption{Linear (lin), exponential-reciprocal (ER), and log-sum-exp (LSE) lower and upper bounds on logistic sigmoid function (softmax for $K=2$ inputs).}
    \label{fig:logistic_bounds}
\end{figure}

\section{LINEARIZED BOUNDS}
\label{sec:lin}

Any tangent plane to a convex lower bound is also a sound lower bound; and any tangent plane to a concave upper bound is also a sound upper bound. A plane tangent to a function $f:\R^K\mapsto \R$ at point $c$ can be described by:

\begin{equation}
    \overline{f_c}(x) = \sum_{j = 1}^{K} \left(\frac{\partial f(c)}{\partial x_j} \left(x_j- c_j\right)\right) + f(c).
\end{equation}

The coefficient of each addend $(x_j - c_j)$ is the partial derivative of $f(x)$ with respect to $x_j$ evaluated at $c$.  As an example, $\frac{\partial L^{\ER}(x)}{\partial x_j}$ can be computed with the chain rule and the results are:
\begin{subequations}\label{eqn:tan_er_LB}
\begin{align}
\frac{\partial L^{\ER}(x)}{\partial x_1}  &= L^{\ER}(x)^2 \cdot \sum^{K}_{j=2} \left(\frac{e^{\tu_j} - e^{\tl_j}}{\tu_j-\tl_j}\right) \label{eqn:tan_er_LB_x1}\\
\frac{\partial L^{\ER}(x)}{\partial x_j}  &= -L^{\ER}(x)^2 \cdot \frac{e^{\tu_j} - e^{\tl_j}}{\tu_j-\tl_j}  \quad \text{for } j \neq 1. \label{eqn:tan_er_LB_xi}
\end{align}
\end{subequations}
Note that while the above linearized bounds derived from $L^\ER$ and the existing linear bound described in Eq.~\eqref{eqn:lin_LB} are both based on the exponential-reciprocal decomposition, there is a key difference: \eqref{eqn:lin_LB} is obtained by composing the linear over-approximations for each decomposition step, while our approach only linearizes \emph{once} after composing the non-linear bounds. 

Linearized bounds for the other nonlinear %lower- and upper- 
bounds in Sections~\ref{sec:ER:non} and \ref{sec:LSE} can be found in App.~\ref{sec:other-lin-bounds}.

While the tangent planes as bounds are strictly less tight than their nonlinear counterparts, these linearized bounds can be useful because they can be integrated in existing bound-propagation frameworks~\citep{singh2019abstract,zhang2018efficient} for NNs, which are designed to efficiently bound the outputs of NNs given a set of inputs. We use them to verify self-attention mechanisms in Section~\ref{sec:appl:attention}

==> Convex Bounds on the Softmax Function/appl.tex <==
\section{APPLICATIONS TO ROBUSTNESS VERIFICATION}
\label{sec:appl}

We present experiments on two robustness verification problems. Our focus remains on showing that the new bounds in Sections~\ref{sec:ER} and \ref{sec:LSE} provide benefits for these tasks, in addition to their theoretical and numerical advantages. 

\subsection{Predictive Uncertainty Estimation}
\label{sec:appl:UQ}

Accurately quantifying uncertainty in predictions is important for calibrating users %conveying an appropriate level of confidence to users 
and for identifying highly uncertain and out-of-distribution examples. Many solutions have been proposed for predictive uncertainty estimation with NNs. %to address the naturally poor ability of NNs to estimate predictive uncertainty. %, notably Bayesian approaches. 
Here we focus on the %simple and 
popular technique of using a \emph{deep ensemble} %an ensemble 
of NNs \citep{lakshminarayanan2017simple,rahaman2021uncertainty}. Verification of the robustness of deep ensembles has not been studied to our knowledge. %\dennis{Not sure whether we need more citations in this paragraph since UQ is not our focus.}

%\dennis{TODO: resolve inconsistent notation and clashing uses of $x, y$ in this section versus previous sections}

To measure the quality of uncertainty estimates, we consider two \emph{proper scoring rules} \citep{gneiting2007strictly}, %metrics, 
negative log-likelihood (NLL) and Brier score. %that are expectations of a and can thus be evaluated on a per-sample basis. That is, 
Given an instance $(x^*, y^*)$ with true label $y^*$ ($x$ now refers to the overall NN input) and predicted probabilities $p_k$ %$\hat{p}(k \given x^*)$ 
for %the instance to belong to 
each class $k = 1, \dots, K$, the scoring rule assigns %we can assign 
a score $S(p, y^*)$. % to $p$. %$S(\hat{p}(\cdot \given x^*), k^*)$ to $\hat{p}(\cdot \given x^*)$. The metric is then computed as the expectation $\mathbb{E}[S(\hat{p}(\cdot \given X), Y)]$ with respect to a (empirical) distribution of $(X, Y)$.
%
To verify the robustness of uncertainty estimates $p$, we bound %our goal is to provide a bound on 
the worst score that can be attained within an $\ell_p$ ball $\mathcal{B}_p(x^*, \epsilon)$ of radius $\epsilon$ around %the given instance 
$x^*$. Using the convention that lower scores are better, we thus wish to solve
\begin{equation}\label{eqn:advScore}
    \max_{x \in \mathcal{B}_p(x^*, \epsilon)} S(p, y^*). %S\bigl(\hat{p}(\cdot \given x), k^*\bigr).
\end{equation}
We formulate \eqref{eqn:advScore} as a concave maximization problem for tractability. Part of this involves expressing $S(p, y^*)$ as, or bounding it from above by, a concave function of $p$. This also suffices for a deep ensemble, where $p$ is the average of probabilities $p^{(m)}$ from the models in the ensemble, since $S(p, y^*)$ or its upper bound will also be concave in $p^{(m)}$.

\paragraph{Negative Log-Likelihood} In the case of NLL, the scoring rule is $S(p, y^*) = -\log p_{y^*}$. While this is not concave in $p$, we can equivalently maximize the linear function 
\begin{equation}\label{eqn:NLL}
    %S\bigl(\hat{p}(\cdot \given x^*), k^*\bigr) = -\log \hat{p}(k^* \given x^*).
    S(p, y^*) = -p_{y^*}.
\end{equation}
%which is linear in $p$.% (i.e., minimize the probability of the correct class).
\begin{comment}
With $\hat{p}$ given by the softmax \eqref{eqn:softmax} of the last-layer activations $x^{(L)}$, this becomes 
\[
    S\bigl(\hat{p}(\cdot \given x^*), k^*\bigr) = \log\left(1 + \sum_{k\neq k^*} e^{x_k^{(L)} - x_{k^*}^{(L)}} \right),
\]
which is a convex log-sum-exp function of $x^{(L)}$. For a tractable maximization problem \eqref{eqn:advScore}, we instead maximize a concave upper bound on the NLL. Such an upper bound can be provided either by $-\log L^\ER(x)$ \eqref{eqn:ER_LB} or by $-\log L^{\lse}(x)$ \eqref{eqn:LSE_LB}, \eqref{eqn:LSE_LB2}. These bounds are concave because the resulting expressions contain compositions of affine functions with $\log$ or just affine functions.
\end{comment}

\paragraph{Brier Score} Here the scoring rule is 
\begin{align}
    %S\bigl(\hat{p}(\cdot \given x^*), k^*\bigr) &= \sum_{k=1}^K \left( \hat{p}(k \given x^*) - \delta_{k=k^*} \right)^2\nonumber\\
    S(p, y^*) = \sum_{k=1}^K \left(p_k - \delta_{k=y^*} \right)^2%\nonumber\\
    %&= (1 - \hat{p}(k^* \given x^*))^2 + \sum_{k\neq k^*} \hat{p}(k \given x^*)^2,
    = (1 - p_{y^*})^2 + \sum_{k\neq y^*} p_k^2,
\end{align}
which is a convex sum-of-squares function of $p$. For tractable optimization, we instead maximize an affine upper bound on the Brier score. For each softmax output $p_k$, we have constant bounds $\ulp_k \leq p_k \leq \olp_k$ from \eqref{eqn:const} (generalized to all $k$, and averaged over models for a deep ensemble). We can then bound the convex univariate functions $(1 - p_{y^*})^2$ and $p_k^2$ by the chords connecting their endpoints, as done throughout Sections~\ref{sec:ER} and \ref{sec:LSE}. The resulting bound can be written as the following affine function of $p$:
\begin{equation}\label{eqn:BrierUB}
    %S\bigl(\hat{p}(\cdot \given x^*), k^*\bigr) \leq -\underbrace{\bigl(2 - \uly_{k^*} - \oly_{k^*}\bigr)}_{\geq 0} y_{k^*} + \sum_{k\neq k^*} (\uly_{k} + \oly_{k}) y_k - \sum_{k=1}^K \uly_k \oly_k + 1,
    %S(p, y^*) \leq -\underbrace{\bigl(2 - \ulp_{y^*} - \olp_{y^*}\bigr)}_{\geq 0} p_{y^*} + \sum_{k\neq y^*} (\ulp_{k} + \olp_{k}) p_k - \sum_{k=1}^K \ulp_k \olp_k + 1,
    S(p, y^*) \leq -2 p_{y^*} + \sum_{k=1}^K (\ulp_{k} + \olp_{k}) p_k - \sum_{k=1}^K \ulp_k \olp_k + 1.
\end{equation}
%which is an affine function of $p$.

Given one of the concave scoring objectives in \eqref{eqn:NLL} or \eqref{eqn:BrierUB}, we relate $p$ to the logits predicted by the network(s) using the lower and upper bounds in Sections~\ref{sec:ER} and \ref{sec:LSE}. The logits play the role of $x$ in these bounds. We then encode the remainder of the NN(s), from input to the logits, using existing convex relaxations, and specifically the triangular linear relaxation \citep{ehlers2017formal} in our experiment. For completeness, the full formulation of \eqref{eqn:advScore} as a concave maximization problem is provided in Appendix~\ref{sec:appl:UQ:formulation}.

For our experiment, we train two deep ensembles with $5$ NNs each on the MNIST dataset using the Uncertainty Baselines\footnote{Available from GitHub repository 
\url{https://github.com/google/uncertainty-baselines}} package in Python. 
% \dennis{Min, please fill in the repo you followed}. 
The architecture of the deep ensemble is given in App.~\ref{sec:arch}. We consider $\ell_\infty$-ball ($\mathcal{B}_\infty(x^*, \epsilon)$) perturbations in \eqref{eqn:advScore}. Input values to the NNs are normalized to between $[0, 1]$. On this scale, we use perturbation bounds $\epsilon = 0.008, 0.012, 0.016$, which correspond to roughly 2, 3, and 4 pixel values. For each of the first $100$ test images, \eqref{eqn:advScore} is solved to bound the score, either NLL or Brier, using different bounds on the softmax. We use CVXPY \citep{diamond2016cvxpy} and its included off-the-shelf solver SCS \citep{scs} to solve these concave problems. We then average over the test images to bound the expected score. 

Table~\ref{tab:UQ} shows the resulting bounds on the expected score. The ``clean'' values are those without perturbation, i.e., $\epsilon = 0$. Recall that the nonlinear bounds denoted $\ER$ and $\lse$ (the two rightmost columns in Table~\ref{tab:UQ}) are both our contributions. While we wished to pair $L^\ER$ with $U^\ER$, using the latter caused the SCS solver to not converge, so we substituted instead the stronger bound $U^{\lse}$. For the LSE pair, we used $L^{\lse*}$ since it suits typical softmax outputs. 
The results indicate that our new nonlinear bounds result in more precise verification of uncertainty quantification than existing linear bounds (represented by $\lin$). In Appendix~\ref{sec:appl:UQ:PGD}, we complement these results with \emph{lower} bounds on worst-case uncertainty estimation scores obtained by using a PGD attack, while in Appendix~\ref{sec:appl:UQ:large}, we show results for an ensemble of larger networks.
%The results continue to support the ranking $\lin < \ER < \lse$ in terms of strength, across $\epsilon$ values and scoring rules.

\begin{table}[h]
\small
\setlength\tabcolsep{3 pt}
\caption{Upper Bounds on Uncertainty Estimation Scores Using Different Softmax Bounds for the MNIST Classifier} \label{tab:UQ}
\begin{center}
\begin{tabular}{lllll}
\textbf{Score (Clean)}   &$\epsilon$ & $L^\lin, U^\lin$ & $L^\ER, U^{\lse}$ & $L^{\lse*}, U^{\lse}$ \\
\hline 
 NLL (0.105)   & 2/256  & 0.265 & 0.261 & \textbf{0.251} \\
        & 3/256  & 0.442 & 0.433 & \textbf{0.420} \\
        & 4/256  & 0.726 & 0.697 & \textbf{0.690} \\ \hline
Brier (0.048)  & 2/256  & 0.138 & 0.134 & \textbf{0.131} \\
        & 3/256  & 0.244 & 0.235 & \textbf{0.234} \\
        & 4/256  & 0.417 & \textbf{0.403} & \textbf{0.403} \\ \hline
%NLL   & 2/256  & 0.25 & 65.2 & 46.8 \\
%        & 3/256  & 0.41 & 35 & 15.4 \\
%        & 4/256  & 0.65 & 11.4 & 4.4 \\ \hline
%Brier   & 2/256  & 0.28 & 65.2 & 46.8 \\
%        & 3/256  & 0.51 & 35 & 15.4 \\
%        & 4/256  & 0.85 & 11.4 & 4.4 \\ \hline
\end{tabular}
\end{center}
\end{table}

We then repeat the same experiment on an ensemble model trained on the CIFAR-10 dataset (architectures can be found in App.~\ref{sec:arch}). Results are shown in Table~\ref{tab:UQ_cifar}.  The results again support the greater strength of the nonlinear bounds over the linear bounds, across $\epsilon$ values and scoring rules. Interestingly, in this case, the $\ER$ lower bound is superior to the $\lse*$ lower bound, suggesting that in practice, $\ER$ and $\lse$ bounds can be complementary. 

\begin{table}[h]
\small
\setlength\tabcolsep{3 pt}
\caption{Upper Bounds on Uncertainty Estimation Scores Using Different Softmax Bounds for the CIFAR-10 Classifier} \label{tab:UQ_cifar}
\begin{center}
\begin{tabular}{lllll}
\textbf{Score (Clean)}   &$\epsilon$ & $L^\lin, U^\lin$ & $L^\ER, U^{\lse}$ & $L^{\lse*}, U^{\lse}$ \\
\hline 
NLL (1.538)   & 2/256  & 2.118 & \bf{2.014} & 2.028 \\
        & 3/256  & 2.569 & \bf{2.433} & 2.474 \\
        & 4/256  & 3.087 & \bf{2.940} & 3.013 \\ \hline
Brier (0.690) & 2/256 & 0.971  & \bf{0.917} & 0.920   \\
        & 3/256  & 1.170 & \bf{1.114} & 1.120  \\
        & 4/256  & 1.367 & \bf{1.324} & 1.329 \\ \hline
\end{tabular}
\end{center}
\end{table}

\paragraph{Timing Results} The average analysis times in seconds per instance using different bounds are shown in Table~\ref{tab:runtime}. The experiments are performed on a cluster equipped with Intel Xeon E5-2637 v4 CPUs. Each job is given one CPU.  

\begin{table}[h]
\caption{Average Runtime in Seconds using Different Bounds}
\label{tab:runtime}
\small
\setlength\tabcolsep{3 pt}
\begin{center}
\begin{tabular}{llll}
\textbf{Dataset} & $L^\lin, U^\lin$ & $L^\ER, U^{\lse}$ & $L^{\lse*}, U^{\lse}$ \\
\hline 
MNIST   & 10.9 & 91.6 & 92.4 \\
CIFAR-10 & 19.5 & 95.3 & 95.5 \\
\hline
\end{tabular}
\end{center}
\end{table}

It must be noted that for this experiment, we are using CVXPY and its off-the-shelf solver SCS, which take time to convert the problems into standard forms and are not customized for them. Hence the runtime results should be interpreted only as confirmation that the convex problems are indeed tractable to solve. In Appendix~\ref{sec:appl:UQ:separate}, we show results from a further over-approximation in which each network in the ensemble is considered separately, which improves computational efficiency.


\subsection{Self-Attention Mechanisms}
\label{sec:appl:attention}

In addition, we consider verifying canonical adversarial robustness properties on neural networks with self-attention mechanisms~\citep{vaswani2017attention}. Self-attention layers involve not only the softmax function, but also bilinear transformations, which are non-trivial to encode as convex optimization problems. Therefore, in this task we instead leverage existing bound-propagation-based methods~\citep{singh2019abstract,zhang2018efficient,Shi2020Robustness}, which already handle bilinear constraints. In particular, we use the CROWN/DeepPoly framework~\citep{singh2019abstract,zhang2018efficient}, a popular bound-propagation method, which requires that each neuron is over-approximated with one linear upper bound and one linear lower bound. Tight convex bounds for bilinear transformation are left as future work. 

\paragraph{MNIST} We train three NNs (named \attSmall, \attMed, and \attBig) with self-attention mechanisms on the MNIST dataset and consider verifying their adversarial robustness against $l_{\infty}$-norm bounded perturbations. The networks are all PGD-trained and vary in size due to different hyper-parameters in the self-attention layers. Details can be found in App.~\ref{sec:arch}. We evaluate on the first 500 test images of the dataset. Inputs to the NNs are again normalized to $[0, 1]$, and we use perturbation bounds 0.016, 0.02, and 0.024, which correspond to roughly 4, 5, and 6 pixel values. 

We consider 4 different linear over-approximations, including the existing linear bounds described in Sec.~\ref{sec:ER:lin} ($\lin$) and %the ones representing the 
tangent planes to the non-linear bounds as discussed in Sec.~\ref{sec:lin}. We consider 3 pairs of tangent planes corresponding to the different nonlinear bounds proposed in this work: $\ER$ is derived from $L^{\ER}$ and $U^{\ER}$; $\lse$ is derived from $L^{\lse}$ and $U^{\lse}$; $\lse*$ is derived from $L^{\lse*}$ and $U^{\lse}$. In all cases we take the tangent plane passing through the midpoint of the softmax input range ($\frac{l + u}{2}$).

\begin{table}[h]
\caption{\% of Instances Certified by Different Softmax Bounds for MNIST classifiers} \label{tab:attention}
\begin{center}
\small
\begin{tabular}{llllll}
\textbf{Net. (Acc.) } &\textbf{Pert.} & \textbf{$\lin$} & \textbf{$\ER$} & \textbf{$\lse$} & \textbf{$\lse*$} \\
\hline
        \attSmall (89.2) & 4/256 & 74.0 & 83.6 & 79.4 & \textbf{84.0} \\ 
        ~ & 5/256 & 67.8 & 79.2 & 73.8 & \textbf{81.2} \\ 
        ~ & 6/256 & 61.2 & 74.6 & 68.6 & \textbf{76.4} \\ \hline
        \attMed (98.2) & 4/256 & 60.0 & 81.2 & 84.4 & \textbf{84.6} \\ 
        ~ & 5/256 & 30.0 & 62.4 & 69.2 & \textbf{71.6} \\ 
        ~ & 6/256 & 11.0 & 34.2 & 39.4 & \textbf{46.0} \\ \hline
        \attBig (99) & 4/256 & 42.0 & 65.0 & 68.6 & \textbf{70.8} \\ 
        ~ & 5/256 & 13.0 & 29.4 & 29.6 & \textbf{41.2} \\ 
        ~ & 6/256 & 1.6 & 6.2 & 3.6 & \textbf{11.6} \\ 
        \hline
\end{tabular}
\end{center}
\end{table}

The percentages of verified instances (out of the 500 test images) using different linear bounds are shown in Table~\ref{tab:attention}. Overall, the new linearized bounds (last 3 columns) result in significantly higher verification precision than $\lin$ does. We believe this is because $\lin$ is obtained by linearization at each step of the decomposition, which results in higher accumulation of approximation errors. Among the new linearized bounds, while $\lse*$ consistently certifies more instances than $\ER$, $\lse$ and $\ER$ are evenly matched with head-to-head wins for both. %solves less instances than $\ER$ for all but one network-perturbation pair. 
Upon further examination, we discover that while $\lse$ is less precise overall, it certifies 9 instances that $\lse*$ is unable to solve and 77 instances that $\ER$ is unable to solve. Overall, the 4 methods combined certify 2628 of the 4500 instances, in contrast to 2572 instances certified by $\lse*$ alone. This suggests the benefit of a portfolio approach. %Heuristic choices in 
Rules for deciding which linearized bounds to use are also an interesting future direction.

\paragraph{SST}
In addition, we perform the same robustness verification task on an NLP transformer model trained on the SST-2 dataset~\citep{socher2013recursive}. SST-2 is a sentiment analysis dataset consisting of movie reviews, where each review is labeled as either positive or negative. In this setting, perturbation is performed on the embedding of the input sentence. The trained transformer obtains 74\% natural accuracy and the robust accuracies verified by different configurations are shown in Table~\ref{tab:attention-sst}. The results further confirm the benefit of the newly proposed linearized bounds (last three columns) over the existing linear bounds ($\lin$). They also highlight the complementary nature of the proposed bounds as unlike in Table~\ref{tab:attention}, $\lse$ is superior to $\lse*$.

\begin{table}[h]
\caption{\% of Instances Certified by Different Softmax Bounds for the SST-2 transformer} \label{tab:attention-sst}
\centering
\small
\begin{tabular}{lllll}
\textbf{Pert. ($\ell_\infty$)} & \textbf{$\lin$} & \textbf{$\ER$} & \textbf{$\lse$} & \textbf{$\lse*$} \\ \hline
0.02 & \textbf{68.8} & \textbf{68.8} & \textbf{68.8} & \textbf{68.8} \\ 
0.04 & \textbf{63.2} & \textbf{63.2} & \textbf{63.2} & \textbf{63.2} \\ 
0.06 & 56.6 & 56.8 & \textbf{57.6} & 57.4 \\ 
0.08 & 51.4 & 52.0 & \textbf{52.4} & \textbf{52.4} \\ 
0.1 & 45.0 & 46.2 & \textbf{47.2} & 46.8 \\ 
0.12 & 39.0 & 39.8 & \textbf{40.6} & \textbf{40.6} \\ 
0.14 & 31.8 & 33.0 & \textbf{34.0} & 33.6 \\ 
0.16 & 26.4 & 26.8 & \textbf{28.2} & 27.2 \\ 
\hline
\end{tabular}
\end{table}


==> Convex Bounds on the Softmax Function/concl.tex <==
\section{CONCLUSION}
\label{sec:concl}

We have provided convex bounds on the softmax function satisfying the hierarchy in \eqref{eqn:ineqChain}, both theoretically and numerically, and used them in certifying the robustness of uncertainty estimators and transformers. Future work could consider the development of more customized algorithms for solving the resulting convex optimization problems, and/or further exploitation of the linearized bounds in Section~\ref{sec:lin} to facilitate scaling to larger networks. We also hope for an even better lower bound from the LSE approach, one that might be provably stronger than $L^\ER$ for $K > 2$ or more smoothly integrate the two bounds $L^{\lse}$, $L^{\lse*}$.

\subsubsection*{Artifact}
Scripts to reproduce the experiments in Sections~\ref{sec:synth} and \ref{sec:appl} can be found at \url{https://github.com/NeuralNetworkVerification/bounding-softmax/tree/aistats}.

==> Convex Bounds on the Softmax Function/definitions.tex <==
\DeclareMathOperator{\se}{SE}
%\newcommand{\se}{s}
\DeclareMathOperator{\lse}{LSE}
\DeclareMathOperator{\sm}{softmax}
\DeclareMathOperator*{\argmax}{arg\,max}
\newcommand{\given}[1][]{\:#1\vert\:}

\newcommand{\ulz}{\underline{z}}
\newcommand{\olz}{\overline{z}}
\newcommand{\uly}{\underline{y}}
\newcommand{\oly}{\overline{y}}
\newcommand{\ulv}{\underline{v}}
\newcommand{\olv}{\overline{v}}
\newcommand{\ulp}{\underline{p}}
\newcommand{\olp}{\overline{p}}
\newcommand{\ulq}{\underline{q}}
\newcommand{\olq}{\overline{q}}
\newcommand{\olse}{\overline{\se}}

\newcommand{\tl}{\tilde{l}}
\newcommand{\tu}{\tilde{u}}
\newcommand{\tx}{\tilde{x}}

\newcommand{\cI}{\mathcal{I}}
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cU}{\mathcal{U}}

\newcommand{\lin}{\mathrm{lin}}
\newcommand{\linShi}{\mathrm{lin}_{\text{S}}}
\newcommand{\ER}{\mathrm{ER}}

\DeclareMathOperator{\lselin}{LSElin}

\DeclareMathOperator{\R}{\mathcal{R}}

\newtheorem{theorem}{Theorem}

%\newcommand{\dennis}[1]{\textcolor{red}{DW: #1}}
\newcommand{\dennis}[1]{}
\newcommand{\andrew}[1]{{\color{red}[Andrew: #1]}}


\newcommand{\attSmall}{\texttt{A$\_$small}\xspace}
\newcommand{\attMed}{\texttt{A$\_$med}\xspace}
\newcommand{\attBig}{\texttt{A$\_$big}\xspace}
\newcommand{\attSST}{\texttt{A$\_$sst}\xspace}

==> Convex Bounds on the Softmax Function/intro.tex <==
\section{INTRODUCTION}
\label{sec:intro}

The softmax function is an indispensable component of multiclass classifiers ranging from multinomial logistic regression models to deep neural networks (NNs). It is most often deployed at the output of a classifier to convert $K$ real-valued scores corresponding to $K$ classes into a probability distribution over the classes. More recently, the softmax is playing an increasing role in intermediate layers as well with the popularization of Transformers~\citep{vaswani2017attention}, whose quintessential component, the (self\nobreakdash-)attention mechanism~\citep{luong2015effective,gehring2017convolutional}, utilizes softmax to compute attention scores.
% \dennis{terminology? citations}, 
% \MW{just added the transformer paper \cite{vaswani2017attention}, will update the text.}

Our main contribution in this paper is to provide convex bounds on the softmax function. More precisely, we derive lower bounds on the outputs of the softmax that are convex functions of the inputs, and upper bounds on the outputs that are concave functions of the inputs (see \eqref{eqn:LU} later). This enables the formulation of convex optimization problems for characterizing ML models with softmax components, particularly in intermediate layers.

We apply our bounds to verification of the robustness of NNs against adversarial input perturbations. %\dennis{more context about adversarial robustness and verification thereof, with citations} 
We consider in particular the quantification of predictive uncertainty for multiclass classifiers, which is typically assessed in terms of accurate estimation of the conditional probability distribution. We are not aware of prior work that directly addresses the robustness of uncertainty estimation metrics, especially for deep ensembles \citep{lakshminarayanan2017simple,rahaman2021uncertainty}, although the works of \citet{bitterwolf2020certifiably,berrada2021make} are related.

Our results are summarized as follows. In Section~\ref{sec:ER}, we first consider an exponential-reciprocal decomposition of the softmax function, used by \citet{Shi2020Robustness,bonaert2021fast} in %their works on 
robustness verification of transformers. While \citet{Shi2020Robustness,bonaert2021fast} limited themselves to linear bounds, we instead derive nonlinear convex bounds (which we refer to as ``ER'') and show that these are tighter than the previous linear bounds (``lin''). We then consider in Section~\ref{sec:LSE} an alternative decomposition in terms of the log-sum-exp (LSE) function, a well-known convex function \citep{boyd2004convex}, and obtain corresponding bounds. We prove that the LSE upper bound is always tighter than the ER upper bound, and that the LSE lower bound is tighter than the ER lower bound for the case of $K=2$ inputs. These analytical results are summarized by the following inequalities, where $L(x)$ and $U(x)$ denote lower and upper bounds that are functions of the input $x$:
\begin{multline}\label{eqn:ineqChain}
    L^\lin(x) \leq L^\ER(x) \underbrace{\leq}_{K=2} L^{\lse}(x) \leq \sm(x)\\
    \leq U^{\lse}(x) \leq U^\ER(x) \leq U^\lin(x).
\end{multline}
For $K > 2$ inputs, while there are instances where $L^\ER(x) > L^{\lse}(x)$, our numerical experiment in Section~\ref{sec:synth} suggests that this does not occur often and that in some regimes, $L^{\lse}$ is tighter by factors of $3$ or more in terms of the mean gap with respect to $\sm(x)$. For the upper bounds, we find that $U^\ER(x)$ improves considerably upon $U^\lin(x)$, which can be rather loose, and $U^{\lse}(x)$ consistently improves upon $U^\ER(x)$ by a further factor of $2$.
In Section~\ref{sec:appl}, we describe experiments on robustness verification of transformers and of uncertainty estimation by deep ensembles. The results provide further evidence of the hierarchy in \eqref{eqn:ineqChain} and of %indicate 
the potential usefulness of the bounds. 

==> Convex Bounds on the Softmax Function/prelim.tex <==
\section{PRELIMINARIES}
\label{sec:prelim}

For an input $x \in \R^K$, the output $p$ of the softmax function is given by
\begin{equation}\label{eqn:softmax}
    p_j = \frac{e^{x_j}}{\sum_{j'=1}^K e^{x_{j'}}} = \frac{1}{1 + \sum_{j'\neq j} e^{x_{j'} - x_j}}, \quad j = 1,\dots,K.
\end{equation}
We work with the second form above, which is preferred in general for numerical stability and also by \citet{bonaert2021fast} for facilitating their approximations (see their Sec.~5.2). To ease notation, we will focus on the first output $p_1$, without loss of generality because of symmetry. Table~\ref{tab:notation} summarizes the notation used in the paper. Based on the second form in \eqref{eqn:softmax}, we accordingly define $\tx_j \coloneqq x_j - x_1$, $j = 1, \dots, K$. In the simplest case of $K = 2$, the softmax reduces to the %univariate 
logistic sigmoid:
\begin{equation}\label{eqn:softmax2}
    p_1 = \frac{1}{1 + e^{\tx_2}} = 1 - p_2.
\end{equation}
%where $x = x_1 - x_2$.

We assume that the set of inputs is contained in the hyper-rectangle defined by $l_j \leq x_j \leq u_j$, $j = 1,\dots,K$, which we write as $l \leq x \leq u$. Our goal is to obtain lower bounds $L(x)$ on $p_1$ that are convex functions of $x$, and upper bounds $U(x)$ that are concave functions of $x$, 
\begin{equation}\label{eqn:LU}
L(x) \leq p_1 \leq U(x).
\end{equation}
Constraints of the form in \eqref{eqn:LU} are desirable in general because they define convex sets of $(x, p_1)$ and can be incorporated into convex optimization problems.

\subsection{Basic Bounds and Constraints}
\label{sec:prelim:constraints}

It can be seen from \eqref{eqn:softmax} that $p_1$ is strictly decreasing in $\tx_j = x_j - x_1$ %increasing in $x_1$ and decreasing in $x_{j}$ 
for $j \neq 1$. We assume that we have bounds $\tl \leq \tx \leq \tu$ on these differences and also define $\tl_1 = \tu_1 \coloneqq 0$ for the trivial case $\tx_1=0$. Given $l \leq x \leq u$, $\tl_j = l_j - u_1$ and $\tu_j = u_j - l_1$ are always valid bounds on $\tx_j$ for $j \neq 1$, %= 2,\dots,K$, 
but we may have tighter bounds as well. The constraints $\tl \leq \tx \leq \tu$ lead to %the following 
lower and upper bounds on $p_1$:
\begin{subequations}\label{eqn:const}
\begin{align}
    \ulp_1 &= \frac{1}{1 + \sum_{j=2}^K e^{\tu_j}} = \frac{1}{\se(\tu)},\label{eqn:const_LB}\\
    \olp_1 &= \frac{1}{1 + \sum_{j=2}^K e^{\tl_j}} = \frac{1}{\se(\tl)},\label{eqn:const_UB}
\end{align}
\end{subequations}
where we have defined %$\tl_j \coloneqq l_j - u_1$ and $\tu_j \coloneqq u_j - l_1$ for $j = 2,\dots,K$, $\tl_1 = \tu_1 = 0$, and 
the sum-of-exponentials function 
$\se(x) \coloneqq \sum_{j=1}^K e^{x_j}.$ 
These are constant bounds in the sense that they are not functions of $x$. The upper bound \eqref{eqn:const_UB} coincides with the bound of \citet[eq.~(6)]{bitterwolf2020certifiably} given the input bounds $\tl$.

We also have the property that $p$ is non-negative and sums to $1$:
\begin{equation}\label{eqn:simplex}
    \sum_{j=1}^K p_j = 1, \qquad p_j \geq 0 \quad \forall j,
\end{equation}
which are linear constraints on $p$. \citet{bonaert2021fast} recognized the benefit of explicitly enforcing \eqref{eqn:simplex} %(although the zonotope refinement process they use to do so is more involved) 
while \citet{Shi2020Robustness} did not use such a constraint.


==> Convex Bounds on the Softmax Function/relWork.tex <==
\subsection{Related Work}
\label{sec:relWork}

Deterministic robustness certification has gained increasing interest in the past few years~\citep{katz2017reluplex,AI2}. Most of the work has focused on verifying properties of the pre-softmax output (e.g.,~\cite{katz2017reluplex,AI2}) for piecewise-linear NNs, while formal reasoning about the softmax outputs themselves has been under-explored. \citet{katz2017reluplex} showed that even the pre-softmax verification problem is computationally inefficient (NP-complete), but a number of approaches based on (linear) abstraction~\citep{singh2019boosting,weng2018towards,zhang2018efficient,gowal2019scalable} and convex optimization~\citep{wong2018provable,dvijotham2018dual} have been proposed to strike a good balance between scalability and precision. We review existing work on NN verification more thoroughly in App.~\ref{sec:nnv-related-work}. 

As mentioned, the softmax function appears in intermediate layers of transformers, and previous works on robustness verification of transformers \citep{Shi2020Robustness,bonaert2021fast} have developed linear lower and upper bounds to approximate the softmax. We review the bounds of \citet{Shi2020Robustness,bonaert2021fast} 
in Section~\ref{sec:ER:lin} as a prelude to deriving provably tighter bounds. \dennis{what else do we want to say about these works?}

Some works have addressed robustness verification of specifications that involve softmax outputs (probabilities) and not just softmax inputs. %(logits). 
\citet{bitterwolf2020certifiably} obtained an upper bound on the maximal probability (i.e., confidence) to verify the robustness of out-of-distribution detectors and train detectors with such guarantees. Their bound coincides with one of our constant bounds in Section~\ref{sec:prelim:constraints}. \citet{berrada2021make} proposed a general framework for probabilistic specifications on the softmax output, where the NN can be stochastic and inputs can have uncertainty. While the uncertainty quantification metrics that we consider fall under their framework, \citet{berrada2021make} do not give explicit formulations for them, let alone implemented algorithms. \dennis{I re-checked the related work section in \citet{berrada2021make}, the other works seem to be for stochastic NNs/inputs and so less related, but would be good for someone else to check.}

\dennis{other related work in the verification literature?}

Bounds on the softmax and log-sum-exp functions have been used in other contexts. For example, \citet{titsias2016one} derived %``one-vs-each'' 
lower bounds on softmax motivated by large-scale classification, \citet{bouchard2007efficient} investigated three upper bounds on log-sum-exp for approximate Bayesian inference, and \citet{nielsen2016guaranteed} used bounds on log-sum-exp to bound information-theoretic measures of mixture models. These bounds, however, do not have the convexity/concavity that we require in the different cases.


==> Convex Bounds on the Softmax Function/synth.tex <==
\section{SYNTHETIC DATA EVALUATION}
\label{sec:synth}

\begin{comment}
\begin{figure*}[t]
\centering
    \begin{subfigure}[b]{0.245\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/synth_lbs_rel_eps10.pdf}
        \caption{$\epsilon = 0.1$, lower bounds}
        \label{fig:synth_lbs_rel_eps10}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.245\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/synth_ER_l_hybrid_l_eps10.pdf}
        \caption{$\epsilon = 0.1$, $L^\ER$ vs.~$L^{\lse}$}
        \label{fig:synth_ER_l_hybrid_l_eps10}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.245\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/synth_ubs_rel_eps10.pdf}
        \caption{$\epsilon = 0.1$, upper bounds}
        \label{fig:synth_ubs_rel_eps10}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.245\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/synth_ER_u_LSE_u_eps10.pdf}
        \caption{$\epsilon = 0.1$, $U^\ER$ vs.~$U^{\lse}$}
        \label{fig:synth_ER_u_LSE_u_eps10}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.245\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/synth_lbs_rel_eps100.pdf}
        \caption{$\epsilon = 1$, lower bounds}
        \label{fig:synth_lbs_rel_eps100}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.245\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/synth_ER_l_hybrid_l_eps100.pdf}
        \caption{$\epsilon = 1$, $L^\ER$ vs.~$L^{\lse}$}
        \label{fig:synth_ER_l_hybrid_l_eps100}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.245\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/synth_ubs_rel_eps100.pdf}
        \caption{$\epsilon = 1$, upper bounds}
        \label{fig:synth_ubs_rel_eps100}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.245\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/synth_ER_u_LSE_u_eps100.pdf}
        \caption{$\epsilon = 1$, $U^\ER$ vs.~$U^{\lse}$}
        \label{fig:synth_ER_u_LSE_u_eps100}
    \end{subfigure}
    \hfill
\caption{Mean gaps of lower bounds (left two columns) and upper bounds (right two columns) for synthetically generated input regions of width $\epsilon = 0.1$ (top row) and $\epsilon = 1$ (bottom row).}
\label{fig:synth}
\end{figure*}
\end{comment}

\begin{figure*}[t]
\centering
    \begin{subfigure}[b]{0.245\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/synth_ubs_rel_d16_high_eps100.pdf}
        \caption{upper bounds, high prob.}
        \label{fig:synth_ubs_rel_d16_high_eps100}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.245\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/synth_ER_u_LSE_u_high0.8_eps100.pdf}
        \caption{$U^\ER$ vs.~$U^{\lse}$, high prob.}
        \label{fig:synth_ER_u_LSE_u_high0.8_eps100}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.245\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/synth_lbs_rel_d16_high_eps100.pdf}
        \caption{lower bounds, high prob.}
        \label{fig:synth_lbs_rel_d16_high_eps100}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.245\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/synth_ER_l_hybrid_l_high0.8_eps100.pdf}
        \caption{$L^\ER$ vs.~$L^{\lse}$, high prob.}
        \label{fig:synth_ER_l_hybrid_l_high0.8_eps100}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.245\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/synth_ubs_rel_d16_low_eps100.pdf}
        \caption{upper bounds, low prob.}
        \label{fig:synth_ubs_rel_d16_low_eps100}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.245\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/synth_ER_u_LSE_u_low0.99_eps100.pdf}
        \caption{$U^\ER$ vs.~$U^{\lse}$, low prob.}
        \label{fig:synth_ER_u_LSE_u_low0.99_eps100}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.245\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/synth_lbs_rel_d16_low_eps100.pdf}
        \caption{lower bounds, low prob.}
        \label{fig:synth_lbs_rel_d16_low_eps100}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.245\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/synth_ER_l_hybrid2_l_low0.99_eps100.pdf}
        \caption{$L^\ER$ vs.~$L^{\lse*}$, low prob.}
        \label{fig:synth_ER_l_hybrid2_l_low0.99_eps100}
    \end{subfigure}
    \hfill
\caption{Mean gaps of upper bounds (left two columns) and lower bounds (right two columns) on softmax output $p_1$ for synthetically generated input regions of width $\epsilon = 1$. In the top/bottom row, the mean $\mu_1$ of $p_1$ is high/low.}
\label{fig:synth}
\end{figure*}


We conduct an experiment using synthetic data to %evaluate and 
compare the tightness of the bounds in Sections~\ref{sec:ER} and \ref{sec:LSE}. For this experiment, we first sample softmax outputs from a $K$-dimensional Dirichlet distribution. To simulate outputs that have varying amounts of probability concentrated on one component, we choose one component of the mean, $\mu_{j_{\max}}$, to be larger than the others, $\mu_{j_{\max}} = \mu_{\max}$, and vary $\mu_{\max}$. More details are in App.~\ref{sec:synth:add}. %the Dirichlet concentration parameters are set to be $\alpha_{j_{\max}} = \alpha_{\max} \geq 1$ for the largest component $j_{\max} \in \{1,\dots,K\}$ and $\alpha_j = 1$ for $j \neq j_{\max}$. We equivalently refer to these distributions in terms of the largest mean component $\mu_{\max} = \alpha_{\max} / \sum_j \alpha_j$. 
We continue to focus on the first softmax output $p_1$ and consider two cases: $j_{\max} = 1$ ($p_1$ has the largest mean) and $j_{\max} \neq 1$ ($p_1$ is among those with small mean). %input regions are created by sampling hypercube centers $m$ from the $K$-dimensional standard Gaussian distribution $\mathcal{N}(0, I_d)$ and 
After sampling a softmax output $p$, we convert it to an %nominal 
input $m$ (i.e., logits). %by taking $m_j = \log(p_j / p_1)$ and centering $m$ by subtracting the mean of the $m_j$'s. 
Bounds on the input region are then set as $l_j = m_j - \epsilon$, $u_j = m_j + \epsilon$ for all $j$, where the width $\epsilon$ is varied. Inputs $x$ are sampled from the uniform distribution over the hypercube $[l, u]$. One hundred ($100$) input regions are generated in this manner, and from each region, $1000$ inputs $x$ are sampled.

For each input $x$, we evaluate %the first softmax output 
$p_1$ \eqref{eqn:softmax} and the following lower and upper bounds: constant $\ulp_1$, $\olp_1$ \eqref{eqn:const}, linear \eqref{eqn:lin}, ER \eqref{eqn:ER}, and LSE \eqref{eqn:LSE}, \eqref{eqn:LSE_LB2}. We leave the linearized bounds of Section~\ref{sec:lin} to App.~\ref{sec:synth:add}. We compute the \emph{mean gap} $p_1 - L(x)$ between the softmax and each lower bound, where the mean is taken over the uniform samples $x$, and similarly the mean gap $U(x) - p_1$ for each upper bound. 

In Figure~\ref{fig:synth}, we plot ratios of mean gaps to focus more on the comparisons between the various bounds. %and less on how the mean gaps vary with other parameters (for example the width $\epsilon$). 
Plots of the mean gaps themselves are in App.~\ref{sec:synth:add}. In Figures~\ref{fig:synth_ubs_rel_d16_high_eps100}, \ref{fig:synth_ubs_rel_d16_low_eps100}, for each input region we divide the mean gap of each upper bound by the mean gap of the constant bound (i.e., $\olp_1 - p_1$). We then plot as a function of $\mu_{\max}$ the mean ratios, taken over the $100$ input regions, as well as the standard errors in the mean. %The dimension $K$ is fixed to $16$; other choices of $K$ are in App.~\ref{sec:synth:add}. 
Figures~\ref{fig:synth_lbs_rel_d16_high_eps100}, \ref{fig:synth_lbs_rel_d16_low_eps100} are the same for the lower bounds. In Figures~\ref{fig:synth_ER_u_LSE_u_high0.8_eps100}, \ref{fig:synth_ER_u_LSE_u_low0.99_eps100}, we take the ratio of the mean gap of $U^\ER$ to that of $U^{\lse}$ and show box plots over the $100$ input regions (whiskers at the $5$th and $95$th percentiles) for different values of $K$. Figures~\ref{fig:synth_ER_l_hybrid_l_high0.8_eps100}, \ref{fig:synth_ER_l_hybrid2_l_low0.99_eps100} are the same for $L^\ER$ versus $L^{\lse}$ and $L^\ER$ versus $L^{\lse*}$ respectively. The top row of Figure~\ref{fig:synth} represents the case $j_{\max} = 1$, where $p_1$ tends to be high, while the bottom row corresponds to $j_{\max} \neq 1$ and low $p_1$. App.~\ref{sec:synth:add} contains plots for values of $K$ and $\epsilon$ other than those indicated in Figure~\ref{fig:synth}. %The width $\epsilon$ is fixed to $1$ in Figure~\ref{fig:synth}; plots for other $\epsilon$ values are in App.~\ref{sec:synth:add}.

We first discuss the %comparison among 
upper bounds (left two columns of Figure~\ref{fig:synth}). %between $L^\ER$ and $L^{\lse}$. 
The linear ER bound $U^\lin$ can be quite loose, as previously suggested by Figure~\ref{fig:logistic_bounds} (see App.~\ref{sec:synth:add} for a possible explanation). In Figure~\ref{fig:synth_ubs_rel_d16_low_eps100}, $U^\lin$ is worse than the constant bound $\olp_1$ by at least an order of magnitude. Thus, moving to the novel nonlinear bound $U^\ER$ can already make a big difference. The bound $U^{\lse}$ provides further improvement, as guaranteed by Theorem~\ref{thm:LSE_ER}, and the improvement factor of around $2$ %from ER to LSE 
is remarkably consistent as a function of $\mu_{\max}$ and $K$. This is particularly evidenced by the narrow distributions of ratios 
in Figures~\ref{fig:synth_ER_u_LSE_u_high0.8_eps100}, \ref{fig:synth_ER_u_LSE_u_low0.99_eps100}.
%$U^\lin$ very loose for $\epsilon = 1$, worse even than constant bound. mean gap ratios fairly consistent vs. $K$, especially ER-LSE upper bound ratio in rightmost column.

Turning now to the lower bounds, %the linear ER bound 
$L^\lin$ is stronger than its counterpart $U^\lin$ in the sense that it improves upon the constant bound $\ulp_1$. The improvement from $L^\lin$ to the novel nonlinear bound 
$L^\ER$ is more marginal. The two LSE bounds $L^{\lse}$ \eqref{eqn:LSE_LB} and $L^{\lse*}$ \eqref{eqn:LSE_LB*} are indeed seen to be complementary as discussed in Section~\ref{sec:LSE}. For $\mu_{\max} \lesssim 0.8$, the largest softmax output does not tend to be that much larger than the others and $L^{\lse}$ is better, whereas for $\mu_{\max} \gtrsim 0.9$, the largest component dominates and $L^{\lse*}$ is better. In the case $j_{\max} \neq 1$ in Figure~\ref{fig:synth_lbs_rel_d16_low_eps100}, the combination of $L^{\lse}$ and $L^{\lse*}$ offer an improvement over $L^\ER$ by a factor ranging from $2.5$--$3$ to much higher. However for $j_{\max} = 1$ and $\mu_{\max} \gtrsim 0.9$ in Figure~\ref{fig:synth_lbs_rel_d16_high_eps100}, $L^{\lse*}$ coincides with $L^\ER$ %(with overwhelming probability since $\mu_{\max}$ is high) 
and there is no improvement. In Figures~\ref{fig:synth_ER_l_hybrid_l_high0.8_eps100}, \ref{fig:synth_ER_l_hybrid2_l_low0.99_eps100}, for $K = 2$ (leftmost box plot), we use \eqref{eqn:LSE_LB2} as the LSE lower bound and the box plots confirm the inequality $L^\ER(x) \leq L^{\lse_2}(x)$ from Theorem~\ref{thm:LSE_ER}. For $K > 2$, the median ratio of mean gaps (orange lines) remains approximately constant, although %. In Figure~\ref{fig:synth_ER_l_hybrid2_l_low0.99_eps100}, the distribution of mean gap ratios widens after $K = 2$ with 
a minority of instances have a ratio less than $1$ in Figure~\ref{fig:synth_ER_l_hybrid_l_high0.8_eps100}. 
%For $K > 2$, the ratio of mean gaps actually increases further, in an average sense in Figures~\ref{fig:synth_lbs_rel_eps10}, \ref{fig:synth_lbs_rel_eps100} and in terms of the medians (orange lines) in Figures~\ref{fig:synth_ER_l_hybrid_l_eps10}, \ref{fig:synth_ER_l_hybrid_l_eps100}. Indeed, $K = 3$ (second box plot from the left in Figures~\ref{fig:synth_ER_l_hybrid_l_eps10}, \ref{fig:synth_ER_l_hybrid_l_eps100}) is the only case in which the mean gap of $L^\ER$ is less than that of $L^{\lse}$, in only a handful of instances. 

%ER-LSE ratios larger than lin-ER ratios. ER-LSE ratio at least 2 and up to 5. 

\dennis{would be best to add the linearized LSE bounds as well}
